Cloud Process Execution Engine - Evaluation of the Core Concepts

In this technical report we describe describe the Domain Specific Language (DSL) of the Workflow Execution Execution (WEE). Instead of interpreting an XML based workflow description language like BPEL, the WEE uses a minimized but expressive set of statements that runs directly on to of a virtual machine that supports the Ruby language.Frameworks/Virtual Machines supporting supporting this language include Java, .NET and there exists also a standalone Virtual Machine. Using a DSL gives us the advantage of maintaining a very compact code base of under 400 lines of code, as the host programming language implements all the concepts like parallelism, threads, checking for syntactic correctness. The implementation just hooks into existing statements to keep track of the workflow and deliver information about current existing context variables and state to the environment that embeds WEE.

==> Images/eval/vpdf2latex <==
#!/usr/bin/env ruby
require 'digest/md5'

begin
  puts "Usage:   #{File.basename($0)} PDF [...] "
  puts "Example: #{File.basename($0)} test1.pdf test2.pdf test3.pdf"
  exit 0
end if ARGV.length < 1

$stdin.sync = true

ARGV.each do |pdf|
  unless File.exist?(pdf)
    puts "#{pdf} does not exist"
  next
end  
print "#{pdf} processing ... "
tmp = Digest::MD5.hexdigest(rand(Time.now).to_s)
`pdftops "#{pdf}" .#{tmp}.ps 1>/dev/null 2>&1`
`ps2eps .#{tmp}.ps .#{tmp}.eps 1>/dev/null 2>&1`
`eps2eps .#{tmp}.eps .#{tmp}1.eps 1>/dev/null 2>&1`
`cp .#{tmp}1.eps "#{pdf.sub(/\.pdf$/,".eps")}"`
`epstopdf .#{tmp}1.eps -o="#{pdf}" 1>/dev/null 2>&1`
`rm .#{tmp}*`
puts "ready"
end  



==> tmp/Makefile <==
TEXC  = latex
PDFC  = pdflatex
BIBC  = bibtex
HTMLC = latex2html -info 0 -split 0 -no-navigation -html_version=4.1
VIEWC = dvips
P2PC  = ps2pdf -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode
PSNUP = psnup -4 -l -m5 -b5
FORCE = touch

BIBS   = $(wildcard *.bib)
TEXD   = $(wildcard *.tex)
LATEXD = $(wildcard *.latex)
LATEXS = $(wildcard *.slide)
BIBTS  = $(patsubst %.bib,%.bib.tmp,$(BIBS))
LATBS  = $(patsubst %.latex,%.latex.bibtmp,$(LATEXD))
PSS    = $(patsubst %.latex,%.ps,$(LATEXD))
DVIS   = $(patsubst %.latex,%.dvi,$(LATEXD))
PDFS   = $(patsubst %.latex,%.pdf,$(LATEXD))
HTMLS  = $(patsubst %.latex,%.html,$(LATEXD))
SLIDES = $(patsubst %.slide,%.slide.pdf,$(LATEXS))
SLIDEV = $(patsubst %.slide,%.view.pdf,$(LATEXS))
SLIDEP = $(patsubst %.slide,%.prn.pdf,$(LATEXS))

all: $(PDFS)
bib: $(PDFS) $(BIBTS) $(LATBS)
ps: $(PSS)
dvi: $(DVIS)
pdf: $(PDFS)
html: ${HTMLS}
slide: $(SLIDES)
slideview: $(SLIDEV)
slideprn: $(SLIDEP)

%.bib.tmp: %.bib
	@cat $< | sed 's/\(howpublished\s\+=\s\+{\)http\([^}]*\)/\1\\url{http\2}/' > $<.tmp
	@mv $<.tmp $<
	@echo Translated $<

%.latex.bibtmp: %.latex
	@$(BIBC) `echo $< | sed 's/\.latex//'`
	@touch $<

%.ps: %.latex
	@$(TEXC) $< 
	@echo "Reparsing for TOC and AUX ..."
	@$(TEXC) $< >/dev/null 2>/dev/null
	@$(VIEWC) `echo $< | sed 's/\.latex/\.dvi/'`
	@rm -f *.log *.dvi *.out

%.prn.pdf: %.slide
	@$(TEXC) $<
	@echo "Reparsing for TOC and AUX ..."
	@$(TEXC) $< >/dev/null 2>/dev/null
	@$(VIEWC) `echo $< | sed 's/\.slide/\.dvi/'`
	@$(PSNUP) `echo $< | sed 's/\.slide/\.ps/'` > `echo $< | sed 's/\.slide/\.prn.ps/'`
	@$(P2PC) `echo $< | sed 's/\.slide/\.prn.ps/'` $@
	@rm -f *.log *.dvi *.out `echo $< | sed 's/\.slide/\.ps/'` `echo $< | sed 's/\.slide/\.prn.ps/'`

%.slide.pdf: %.slide
	@$(TEXC) $<
	@echo "Reparsing for TOC and AUX ..."
	@$(TEXC) $< >/dev/null 2>/dev/null
	@$(VIEWC) `echo $< | sed 's/\.slide/\.dvi/'`
	@$(P2PC) `echo $< | sed 's/\.slide/\.ps/'` $@
	@rm -f *.log *.dvi *.out `echo $< | sed 's/\.slide/\.ps/'`

%.view.pdf: %.slide
	@$(TEXC) $<
	@echo "Reparsing for TOC and AUX ..."
	@$(TEXC) $< >/dev/null 2>/dev/null
	@$(VIEWC) `echo $< | sed 's/\.slide/\.dvi/'`
	@$(P2PC) `echo $< | sed 's/\.slide/\.ps/'` $@
	@rm -f *.log *.dvi *.out `echo $< | sed 's/\.slide/\.ps/'`

%.pdf: %.latex ${TEXD}
	@$(PDFC) $< 
	@echo "Reparsing for TOC and AUX ..."
	@$(PDFC) $< >/dev/null 2>/dev/null
	@rm -f *.log *.out  

%.html: %.latex
	@$(HTMLC) $< 
	@cat `echo $< | sed 's/\.latex//'`/`echo $< | sed 's/\.latex//'`.html | sed 's/CELLPADDING=[^> ]*/CELLPADDING=0 CELLSPACING=0/' > `echo $< | sed 's/\.latex//'`/eTestXXXXX.html
	@mv `echo $< | sed 's/\.latex//'`/eTestXXXXX.html `echo $< | sed 's/\.latex//'`/`echo $< | sed 's/\.latex//'`.html
	@rm `echo $< | sed 's/\.latex//'`/index.html

force: $(LATEXD)
	@$(FORCE) $< 

clean:
	@rm -f *.ps *.dvi *.pdf *.bak *.log *.aux *.toc *.out *.bbl *.blg
	@echo
	@echo "   Cleaned Directory!"
	@echo

